Boosting Latent Diffusion with Flow Matching

Visual synthesis has recently seen significant leaps in performance, largely due to breakthroughs in generative models. Diffusion models have been a key enabler, as they excel in image diversity. However, this comes at the cost of slow training and synthesis, which is only partially alleviated by latent diffusion. To this end, flow matching is an appealing approach due to its complementary characteristics of faster training and inference but less diverse synthesis. We demonstrate that introducing flow matching between a frozen diffusion model and a convolutional decoder enables high-resolution image synthesis at reduced computational cost and model size. A small diffusion model can then effectively provide the necessary visual diversity, while flow matching efficiently enhances resolution and detail by mapping the small to a high-dimensional latent space. These latents are then projected to high-resolution images by the subsequent convolutional decoder of the latent diffusion approach. Combining the diversity of diffusion models, the efficiency of flow matching, and the effectiveness of convolutional decoders, state-of-the-art high-resolution image synthesis is achieved at $1024^2$ pixels with minimal computational cost. Further scaling up our method we can reach resolutions up to $2048^2$ pixels. Importantly, our approach is orthogonal to recent approximation and speed-up strategies for the underlying model, making it easily integrable into the various diffusion model frameworks.

==> figures/autoencoder.tex <==
\begin{figure*}
    \centering
    % \vspace{-0.5cm}
    \includegraphics[width=0.9\textwidth]{figures/img/autoencoder_perform.pdf}
    % \vspace{-0.5cm}
    \caption{Comparison between reconstructed images (middle $256^2$ and right column $2048^2$) and their high-resolution original input (left column) using the pre-trained autoencoder.  We can observe that the (i) pre-trained autoencoder is able to encode and decode images at different scales. (ii) It cannot reconstruct faces correctly in low resolution. (iii) The artifacts diminish with a higher resolution. Best viewed when zoomed in.
    }
    \label{fig:auto_visual}
    % \vspace{-10pt}
\end{figure*}

==> figures/sup/chaining-2k.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.5cm}
    \includegraphics[width=\textwidth]{figures/img/128->2k.pdf}
    \caption{\todo{Placeholder. Insert another chaining image here in full resolution.}}
    \label{fig:sup:chaining-2k}
    % \vspace{-20pt}
\end{figure*}


==> figures/sup/ldm32_generations.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/sup/ldm32_generations.png}
    \caption{\todo{Placeholder. Insert our figure here with low-res vs high-res for LDM32 -> 1k.}}
    \label{fig:sup:ldm32-generations}
\end{figure}


==> tables/laion-eval.tex <==
\begin{table*}[t]
    
    \centering   
    \begin{tabular}{l||cccc|cccc}
    \toprule
      & \multicolumn{4}{c|}{FacesHQ}                                           & \multicolumn{4}{c}{LHQ} \\
        Model       & SSIM$\uparrow$   & PSNR$\uparrow$   & FID$\downarrow$ & p-FID$\downarrow$   & SSIM$\uparrow$       & PSNR$\uparrow$       & FID$\downarrow$ & p-FID$\downarrow$  \\
        \midrule
        $L1$        & \textbf{0.86}     & \textbf{31.78}    & 4.52              & 6.51     & \textbf{0.72}         & \textbf{26.99}        & 4.88    & 6.54       \\
        \midrule
        CFM (\textit{ours}) & 0.82  & 30.40     & \textbf{1.36}     & \textbf{1.62}     & \underline{0.69}     & 25.69                 & \textbf{2.27}   & \textbf{2.38}   \\
    \bottomrule
    \end{tabular}
    \caption{Quantitative results of combining our method with  results for $L1$ and $L2$ regression, diffusion-based (DM) similar to \cite{saharia2022_SR3}, Flow Matching (\textit{FM}) \cite{lipman2023flow}, and our Coupling Flow Matching (\textit{CFM}) on 5k samples from FacesHQ and LHQ high-resolution datasets, respectively. \todo{make sure to replace SR3 in the text. We use it for two cases: pixel space (legit SR3) and replace our FM module with theirs, denoted now as DM now; add what p-FID is}}
    \vspace{-3mm}
    % $256 \times 256 \rightarrow 1024 \times 1024$ super-resolution results.
    \label{tab:upsample_model}
\end{table*}

==> tables/laion_sampling_64.tex <==
\begin{table}[tbph]
    \setlength\tabcolsep{10.pt}
    
    \centering   
\begin{tabular}{c||c|c|c|c}
    \toprule
    \textbf{Models}  & \textbf{CLIP} $\uparrow$ & \textbf{FID} $\downarrow$  & \textbf{p-FID} $\downarrow$  &\textbf{time} \textit{s} $\downarrow$ \\
    \midrule
    LCM-LoRA (SD1.5) \cite{luo2023lcm} + CFM    & 23.50   & 36.83    & 31.02 & 0.48\\
    SD15+diffusion(NFE4)     & 25.68    &  26.53  & 25.20 & 2.72 \\
    SD15+CFM (NFE4)          & 26.16   &  21.61  & 15.83 & 2.72\\
    SD15+diffusion(NFE40)    & 26.05   &  22.29  & 16.36 & 3.16 \\
    SD15+CFM (NFE40)         & 26.14   &  21.67  & 15.96 & 3.16\\
    LCM-LoRA-SDXL \cite{luo2023lcm}            & 24.51   &  28.98  & 24.00 & 1.83\\
    
    \midrule
    SD15+diffusion(NFE40) 50k   & 26.03   &  10.38  & 10.51 & \\
    SD15+CFM (NFE40)  50k       & 26.09   &  10.09  & 10.13 & \\
    \bottomrule
\end{tabular}
\caption{Laion sampling evaluation $512^2 \rightarrow 1024^2$}
\vspace{-3mm}
\label{tab:laion_sampling_64}
\end{table}


==> tables/model_size_ablation.tex <==
\npdecimalsign{.}
\nprounddigits{2}
\begin{table}[t]
    \setlength\tabcolsep{1.5pt}
    \centering
    
    \begin{tabular}{l||ccc||ccc}
    \toprule
      & \multicolumn{3}{c|}{Big (306M)} & \multicolumn{3}{c}{Small (113M)} \\
    \textbf{Model} & \textbf{SSIM} $\uparrow$ & \textbf{PSNR} $\uparrow$ & \textbf{FID} $\downarrow$ & \textbf{SSIM} $\uparrow$ & \textbf{PSNR} $\uparrow$ &  \textbf{FID} $\downarrow$ \\ 
            \midrule
                FM & 0.59  & 22.90 & 11.22 & 0.59   & 22.84  & 10.90\\

                CFM-400 & 0.59  & 22.72 & 6.30 & 0.59   & 22.87  & 6.38\\
                
                CFM-200 & 0.60  & 22.98 & 4.92 & 0.60   & 23.02  & 5.20\\
                % \midrule
                
                % \midrule
                

            \bottomrule
    \end{tabular}
    \caption{LHQ ablation for $256^2 \rightarrow 1024^2$ super-resolution results. 
    }
    \label{tab:model-size-ablation}
\end{table}
